Analysis of Moral Judgement on Reddit

Moral outrage has become synonymous with social media in recent years. However, the preponderance of academic analysis on social media websites has focused on hate speech and misinformation. This paper focuses on analyzing moral judgements rendered on social media by capturing the moral judgements that are passed in the subreddit /r/AmITheAsshole on Reddit. Using the labels associated with each judgement we train a classifier that can take a comment and determine whether it judges the user who made the original post to have positive or negative moral valence. Then, we use this classifier to investigate an assortment of website traits surrounding moral judgements in ten other subreddits, including where negative moral users like to post and their posting patterns. Our findings also indicate that posts that are judged in a positive manner will score higher.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> awry.tex <==
\section{Conversations Gone Awry}
An interesting avenue of work that has been investigated recently is the ability to preempt a conversation if you know further discussion will result in a personal attack \cite{zhang_2018_ConversationsGoneAwry, chang_2019_TroubleHorizonForecasting}. 
This differs from other frameworks that try to detect these personal attacks after they have already happened.
In this task two datasets have been used one from Wikipedia discussion pages and the other from the subreddit \texttt{r/ChangeMyView}.
Each dataset consists of a back and forth conversation between users with some ending in a personal attack.
With this task in mind we wondered whether our asshole predictor could be transferred and used to predict these personal attacks as well.
The judgements user give on \texttt{r/AmITheAsshole} can be viewed as a form personal attacks when someone calls the original poster an asshole, since the user is expected to explain and give reasoning as to why this person is an asshole.
Due to this we wondered whether our classifier could be used on the conversations gone awry dataset to perform the same prediction task.

There are three different methods that have been used to solve this problem so far.
The first method uses a TF-IDF weighted bag-of-words representation extracted from the first comment-reply pair in the conversations.
The second method, called Awry, uses the first comment-reply pair of the conversation and extracts pragmatic features to use. 
These pragmatic features include 38 different politeness strategies and 12 different prompt types.
The final model is called CRAFT (Conversational Recurrent Architecture for Forecasting) and is the current state of the art for this problem.
CRAFT consists of two parts, a pre-trained hierarchical recurrent encoder-decoder \cite{sordoni_2015_HierarchicalRecurrentEncoderDecoder} and a prediction component that is just a multilayer perceptron with three fully-connected layers.
One major difference of the CRAFT model is that it works in an online fashion. This allows it to process comments in order and gain a context of what is happening in the conversation to signal it will de-reail.
Due to this factor the authors of CRAFT re-implemented the prior methods to also handle the comments in an online manner.

For our method we utilize our AITA classifier in both ways for this task. We first experiment with just using the second comment in each of the conversations. If our classifier predicts they are calling the original poster an asshole then we believe the conversation will de-rail. Otherwise, our prediction believes the conversation will proceed normally.
We also modified our model to stream comments in an online fashion as was done in the previous works.
Once our model makes a prediction that someone is an asshole we stop predicting and believe the conversation will end in a personal attack. Otherwise we force the model to continue down through all the comments and continue predicting.

We present our results in Table \ref{tab:awry}. 
The results for our AITA classifier using just the second comment performs almost as well as the original Awry method on the Wikipedia talk pages. It does outperform a simple bag-of-words model. Part of the reason for it's performance is that it does not guess many of the conversations to de-rail. We can see a degradation in performance when we shift to the online model. In our online version our model ends up detecting too many of the posts as calling the other user an asshole to signal the derailment. This stands in contrast to all of the other methods that saw an increase in performance when shifting to an online version.
Overall our model does not seem to generalize to this other task very well. Our results do show that some of the language tendencies between calling someone an asshole and a conversation derailing may overlap. 



\begin{table*}[h]
\begin{tabularx}{\linewidth}{l XXXXX | XXXXX}
\toprule
      &  \multicolumn{5}{c}{Wikipedia Talk Pages} & \multicolumn{5}{c}{Reddit CMV} \\
      \cmidrule{3-5} \cmidrule{8-10}
    \textbf{Model} & \textbf{A} & \textbf{P} & \textbf{R} & \textbf{FPR} & \textbf{F1} & \textbf{A} & \textbf{P} & \textbf{R} & \textbf{FPR} & \textbf{F1} \\
    \midrule
    BoW & 56.5 & 55.6 & 65.5 & 52.4 & 60.1 & 52.1 & 51.8 & 61.3 & 57.0 & 56.1 \\
    Awry & 58.9 & 59.2 & 57.6 & 39.8 & 58.4 & 54.4 & 55.0 & 48.3 & 39.5 & 51.4 \\
    Cumul. BoW & 60.6 & 57.7 & 79.3 & 58.1 & 66.8 & 59.9 & 58.8 & 65.9 & 46.2 & 62.1 \\
    Sliding Awry & 60.6 & 60.2 & 62.4 & 41.2 & 61.3 & 56.8 & 56.6 & 58.2 & 44.6 & 57.4 \\
    CRAFT & 66.5 & 63.7 & 77.1 & 44.1 & 69.8 & 63.4 & 60.4 & 77.5 & 50.7 & 67.9 \\
    AITA & 57.3 & 57.9 & 57.3 & 14.4 & 57.5 & 53.3 & 53.3 & 53.3 & 22.4 & 53.3 \\
    AITA Online & 54.8 & 58.6 & 54.8 & 66.8 & 56.6 & 52.1 & 55.9 & 52.1 & 44.1 & 53.9 \\
    
%Personal Attack & 67.53 & 50.0 & 33.76 & 40.31 & NA \\

\bottomrule
\end{tabularx}
\caption{Comparison of our AITA classifier used on the conversations gone awry dataset. Evaluation is done using accuracy, precision, recall, false positive rate, and F1 score.}
\label{tab:awry}
\vspace{-0.5cm}
\end{table*}

==> figs/aita-example.tex <==
\begin{figure}[ht!]
 \centering    

    \subfloat[]{\includegraphics[width=0.43\textwidth]{figs/aita-post-example.png}}

     \subfloat[]{\includegraphics[width=0.43\textwidth]{figs/aita-respons-example.png}}

    \vspace{-0.25cm}
 \caption{\label{fig:aita-ex} Example of (a) a post title and (b) a comment in the \texttt{r/AmItheAsshole} subreddit. Not displayed is the content of the post, i.e., the description of the situation.}
\end{figure}

==> related_work.tex <==
\section{Related Work}

% o	Section 2. Related work. 
% 	History of Netflix competition (L07)
% 	The related work each team reviewed (Proposal)


The dynamics of discussion have been studied in many ways. One common way of doing so is analyzing the sentiment of the text in question. To do so, the text must first be embedded as a low dimensional feature vector. Then, given the sentiment of the text, e.g., positive or negative, one can train a classifier over the feature vectors, using the sentiment as the labels. As such, we discuss relevant text embedding methods, as follows.

% word2vec \cite{mikolov2013efficient} uses a skip-gram model to perform its embedding.  only words. did not work well when combining embeddings to get paragraph embeddings.

Many text embedding methods focus on obtaining feature vectors for single words at a time \cite{voorhees1999natural, mikolov2013efficient, pennington2014glove, peters2018deep}. However, it is also important to study groups of words (sentences, paragraphs) \cite{mitchell2010composition, maas2011learning, le2014distributed}. While simply combining feature vectors of each individual word in a sentence is one way to obtain group-level embeddings, this is often lacking. Doc2Vec \cite{le2014distributed} introduces an approach to embed groups of words at a time. It does so using a similar approach to its predecessor, word2vec \cite{mikolov2013efficient}. However, Doc2Vec is also able to take into account the word order, and better embeds semantically similar words to each other. Several approaches have been proposed since, including many deep learning-based models \cite{kim2014convolutional, tai2015improved, lai2015recurrent, joulin2016bag, devlin2018bert}. However, BERT \cite{devlin2018bert} is the current state-of-the-art. It uses a multilayer bidirectional Transformer encoder to learn the representation of a sequence of text, making it applicable to both words and groups of words. 

% ELMo \cite{peters2017semi}


The main drawback of sentiment analysis in the context of discussions, however, is that they do not account for how a given piece of text is responding to another. Presumably, the words people use in reaction to a situation depend on the morality of that situation. One approach does consider the response dynamic, though it does so in a general sense and not specifically for morality, described below.

% Different types of ``conversational archetypes'' \cite{guimaraes2019analyzing}
Guimar\~{a}es et al. \cite{guimaraes2019analyzing} are interested in understanding different types of discussions that occur in the subreddits \texttt{r/politics} and \texttt{r/worldnews}. They propose four ``conversational archetypes'' that describe how a discussion progresses, and aim to test 10 hypotheses associated with them. For example, they hypothesize that ``Harmonious'' discussions, ones in which all the posts are not marked as ``controversial'' by Reddit standards, have high positive sentiment scores. 






==> tables/asshole_class_labels.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
Abbreviation & Meaning             \\ \hline
NTA          & Not the Asshole     \\ %\hline
YTA          & You're the Asshole  \\ %\hline
NAH          & No assholes here    \\ %\hline
ESH          & Everyone sucks here \\ \hline
\end{tabular}
\caption{The four judgements that users can pass on the subreddit r/AmItheAsshole.}
\label{tab:abbreviations}
\vspace{-0.5cm}
\end{table}

==> tables/classification-results_new.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{c| llll}
    \toprule
    \textbf{Method} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
    \midrule
      Doc2Vec   & 65.92 $\pm$ 0.04 & 61.22 $\pm$ 0.15 & 13.5 $\pm$ 0.09 & 22.1 $\pm$ 0.09  \\
     BERT Embedding     & 70.10 $\pm$ 0.07 & 64.28 $\pm$ 0.2 & 36.96 $\pm$ 0.14 & 46.96 $\pm$ 0.08 \\
     Multinomial Naive Bayes & 72.12 $\pm$ 0.17 & 62.58 $\pm$ 0.17 & 55.22 $\pm$ 0.07 & 58.66 $\pm$ 0.05 \\
     Asshole BERT & 89.03 $\pm$ 0.13 & 85.57 $\pm$ 0.18 & 83.48 $\pm$ 0.27 & 84.51 $\pm$ 0.17 \\

     %\midrule
     %NB-Matrix-Sum-1000D & 0.641 $\pm$ 0.001 & 0.499 $\pm$ 0.0013 & 0.59 $\pm$ 0.001 & 0.54 $\pm$ 0.001 \\
     %NB-Matrix-Average-1000D & 0.667 $\pm$ 0.001 & 0.77 $\pm$ 0.005 & 0.102 $\pm$ 0.0 & 0.18 $\pm$ 0.001 \\
     %NB-Matrix-Min-1000D & 0.657 $\pm$ 0.001 & 0.852 $\pm$ 0.002 & 0.054 $\pm$ 0.001 & 0.101 $\pm$ 0.001 \\
     %NB-Matrix-Max-1000D & 0.676 $\pm$ 0.001 & 0.711 $\pm$ 0.003 & 0.162 $\pm$ 0.001 & 0.264 $\pm$ 0.001 \\
     %\midrule
     %LogR-Sum-2000 & 0.687 $\pm$ 0.001 & 0.657 $\pm$ 0.002 & 0.264 $\pm$ 0.001 & 0.377 $\pm$ 0.0 \\
    %NB-Sum-2000 & 0.654 $\pm$ 0.001 & 0.515 $\pm$ 0.001 & 0.603 $\pm$ 0.001 & 0.556 $\pm$ 0.001 \\
    %RF-Sum-2000 & 0.72 $\pm$ 0.001 & 0.69 $\pm$ 0.002 & 0.395 $\pm$ 0.001 & 0.503 $\pm$ 0.001 \\
    %LogR-Average-2000 & 0.702 $\pm$ 0.001 & 0.662 $\pm$ 0.001 & 0.342 $\pm$ 0.001 & 0.451 $\pm$ 0.0 \\
    %NB-Average-2000 & 0.68 $\pm$ 0.001 & 0.766 $\pm$ 0.003 & 0.153 $\pm$ 0.001 & 0.255 $\pm$ 0.001 \\
    %RF-Average-2000 & \textbf{0.775 $\pm$ 0.001} & 0.703 $\pm$ 0.001 & \textbf{0.645 $\pm$ 0.002} & \textbf{0.673 $\pm$ 0.001} \\
    %LogR-Min-2000 & 0.718 $\pm$ 0.001 & 0.695 $\pm$ 0.001 & 0.379 $\pm$ 0.001 & 0.49 $\pm$ 0.001 \\
    %NB-Min-2000 & 0.669 $\pm$ 0.001 & \textbf{0.873 $\pm$ 0.003} & 0.09 $\pm$ 0.001 & 0.163 $\pm$ 0.001 \\
    %RF-Min-2000 & 0.756 $\pm$ 0.001 & 0.694 $\pm$ 0.001 & 0.568 $\pm$ 0.002 & 0.625 $\pm$ 0.001 \\
    %LogR-Max-2000 & 0.698 $\pm$ 0.001 & 0.656 $\pm$ 0.001 & 0.33 $\pm$ 0.001 & 0.439 $\pm$ 0.0 \\
    %NB-Max-2000 & 0.689 $\pm$ 0.002 & 0.697 $\pm$ 0.003 & 0.235 $\pm$ 0.001 & 0.351 $\pm$ 0.001 \\
    %RF-Max-2000 & 0.731 $\pm$ 0.001 & 0.669 $\pm$ 0.002 & 0.497 $\pm$ 0.002 & 0.57 $\pm$ 0.002 \\
     \bottomrule
    \end{tabular}
    \caption{Classification results on the AITA dataset. All methods used five-fold cross-validation and report the mean values along with the standard deviations.}
    \label{tab:binary_classification_results}
\end{table*}

==> tables/co-occurrence_operators.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
Operator & Meaning             \\ \hline
Sum      & $\sum\limits_{i=1}^{n} x_i$              \\ %\hline
Average  & $\sum\limits_{i=1}^{n}  {x_i}{n}$           \\ %\hline
Max      & $Max(x_1, ..., x_n)$                    \\ %\hline
Min      & $Min(x_1, ..., x_n)$ \\ \hline
\end{tabular}
\caption{Operators for $combine(x_1, ... x_n)$.}
\label{tab:operators}
\vspace{-0.5cm}
\end{table}

==> tables/prediction_analysis.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|l|lllll|}
\hline
Method & TP & TP + FP & TP + FN & Precision & Recall  \\ 
\hline
Doc2Vec & 187 & 338 & 1,566 & 0.553 & 0.119   \\
BERT & 574 & 956 & 1,566 & 0.6 & 0.367 \\
Doc2Vec $\cap$ BERT & 87 & 180 & 1,566 & 0.483 & 0.0556 \\


\hline

\end{tabular}
\caption{Detailed statistics regarding predictions made by Doc2Vec and BERT. Doc2Vec $\cap$ BERT indicates the overlap of predictions made by both methods.}
\label{tab:pred-analysis}
\end{table*}

==> tables/relationship_contingency_tables.tex <==
\begin{table}

\centering
% relationship_advice
\begin{tabular}{ccc}
 & \texttt{r/relationship\_advice} & \\
\toprule
&\textbf{Non-Asshole}&\textbf{Asshole}\\
\textbf{Male}&58,350&28,806\\
\textbf{Female}&60,468&21,927\\
\bottomrule
\end{tabular}

\vspace{0.5cm}

%relationships
\begin{tabular}{ccc}
& \texttt{r/relationships} & \\
\toprule
&\textbf{Non-Asshole}&\textbf{Asshole}\\
\textbf{Male}&151,141&80,618\\
\textbf{Female}&226,042&82,219\\
\bottomrule
\end{tabular}
\caption{Contingency tables showing the number of non-asshole and asshole judgements for each gender in \texttt{r/relationship\_advice} and \texttt{r/relationships}.}

\label{tab:relationship-contingency}
\end{table}











%\begin{table}[]
%\parbox{.45\linewidth
%    \centering
 %   \begin{tabular}{c|c|c}
 %   
 %        & Non-Asshole  & Asshole  \\
 %      Male  &  &  \\
%        Female  &  & \\
%    
%    \end{tabular}
%    \caption{relationships}
%    }
%    
%\parbox{.45\linewidth
%    \centering
%    \begin{tabular}{c|c|c}
%    
%         & Non-Asshole  & Asshole  \\
%       Male  &  &  \\
%        Female  &  &
%        
%    \end{tabular}
%    
%    \caption{}
%    }
%    \label{tab:relationship-contingency}
%\end{table}

==> tables/subreddit_user_stats.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l  llll}
    \toprule
        \textbf{Subreddit} & \textbf{\# NTA} & \textbf{\# YTA}  & \textbf{\# Users} \\
        \midrule
        relationship\_advice & 154,029 &	54,855 &	2,647  \\
         dating\_advice &	63,095 &	27,628 &	1,578 \\
         legaladvice & 226,436 & 44,731 &  2,152 \\
         dating & 18,271 & 7,299  & 637 \\
         confessions & 19,507 & 10,706 &  1,043 \\
         TrueOffMyChest & 20,446 & 9,914 &  1,142 \\
         offmychest & 14,466 & 4,084 &  1,029 \\
         changemyview & 225,662 & 150,378 &  2,678 \\
         CasualConversation & 175,008 & 45,601 &  2,309 \\
         \bottomrule
    \end{tabular}
    \caption{Breakdown statistics for each subreddit for 2018. This captures only users that have been judged at least 50 times across these subreddits.}
    \label{tab:subreddit_user_stats}
\end{table}
